Project and Conquer: Fast Quantifier Elimination for Checking Petri Net Reachability

We propose a method for checking generalized reachability properties in Petri nets that takes advantage of structural reductions and that can be used, transparently, as a pre-processing step of existing model-checkers. Our approach is based on a new procedure that can project a property, about an initial Petri net, into an equivalent formula that only refers to the reduced version of this net. Our projection is defined as a variable elimination procedure for linear integer arithmetic tailored to the specific kind of constraints we handle. It has linear complexity, is guaranteed to return a sound property, and makes use of a simple condition to detect when the result is exact. Experimental results show that our approach works well in practice and that it can be useful even when there is only a limited amount of reductions.

==> macros.tex <==
\let\proof\relax
\let\endproof\relax
\let\example\relax
\let\endexample\relax

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{lineno}
\linenumbers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amssymb,amsmath,amsthm}
\usepackage{mathtools}

\usepackage{graphicx}
%\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[linesnumbered,ruled,vlined,noend]{algorithm2e}

\usepackage{booktabs}
\usepackage{array}
\usepackage{multirow,makecell}
\usepackage{pgfplots}
\usepackage{url}
\usepackage{float}
\usepackage{stmaryrd}
%\usepackage{scalerel}
\usepackage{xfp}

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{4}
\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-12\p@ \@plus -4\p@ \@minus -4\p@}%
                       {-0.5em \@plus -0.22em \@minus -0.1em}%
                       {\normalfont\normalsize\bfseries\boldmath}}
\makeatother
\usepackage{bookmark}

\usepackage{hyperref}
\usepackage{siunitx}
\renewcommand{\labelitemi}{$\bullet$}
\renewcommand\UrlFont{\color{blue}\rmfamily}
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations
}

\usepackage{arydshln}
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}

\newcommand{\ratioc}[2]{${#1}$ && ${#2}$ && $\times$\fpeval{trunc({#1} / {#2}, 2)}}
\newcommand{\ratiod}[2]{${#1}$ && ${#2}$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{todonotes}
\newcommand{\SDZ}[1]{\todo{SDZ: {#1}}}
\newcommand{\NA}[1]{\todo{NA: {#1}}}
\newcommand{\fv}[1]{\ensuremath{\mathit{fv}({#1})}}
\newcommand{\succs}[1]{\ensuremath{\mathord{\downarrow}{#1}}}
\newcommand{\preds}[1]{\ensuremath{\mathord{\uparrow}{#1}}}
\newcommand{\caesar}{\textsc{c{\ae}sar.bdd}}
\newcommand{\conc}{\ensuremath{\mathbin{\|}}}
\newcommand{\Conc}{\ensuremath{\mathrm{C}}}
\newcommand{\bconc}{\mathop{\mathcal{C}}}
\newcommand{\bind}{\mathop{\bar{\mathcal{C}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\red}{\mathbin{{\rightarrow}\!{\bullet}}}
\newcommand{\agg}{\mathbin{{\circ}\!{\rightarrow}}}
% \newcommand{\mred}{\mathbin{{\bullet}\!{\leftarrow}}}
% \newcommand{\magg}{\mathbin{\agg}}
%\newcommand{\mboth}{\mathbin{\leftrightarrow}}
\newcommand{\lvl}[1]{\mathrm{lvl}({#1})}

%\newcommand{\maseq}[1]{\underline{#1}}
\newcommand{\maseq}[1]{\lfloor {#1} \rfloor}

\newcommand{\comma}{\mathbin{\raisebox{0.2ex}{\textbf{,}}}}
% \newcommand{\comma}{\mathbin{\textbf{,}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\myplies}{\mathop{\Rightarrow}}
\newcommand{\TIMEOUT}{\colorbox{red!10!white}{---}}
\newcommand{\UNAV}{\textsf{X}}

\newcommand{\reduc}{\vartriangleright}
\newcommand*{\defeq}{\triangleq} %% {\stackrel{\text{def}}{=}}

%% \newcommand{\marking}[2]{{#1}{\ast}{#2}}
%%
% use \marking{{p0}{1}{p3}{4}{p6}{1}} to obtain p0*1 p3*4 p6*1
% \marking has one parameter that is an even-length list of
% {place}{int}
%
\newif\ifmarkingSep
\newcommand*{\marking}[1]{%
  \relax
  \markingSepfalse
  \markingScan#1\relax\relax
}
\newcommand{\markingScan}[2]{%
  \ifx\relax#1\empty
  \else
    \ifmarkingSep
      {\,}\relax
    \else
      \markingSeptrue
    \fi
    {#1}{\ast}{#2}\relax
    \expandafter\markingScan
  \fi
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def \rightarrowfill{\m@th\mathord{\smash-}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash-}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\rightarrow}
\makeatother

\makeatletter
\def \Rightarrowfill{\m@th\mathord{\smash-}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash-}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\Rightarrow}
\makeatother

\makeatletter
\def \rightarrowfill{\m@th\mathord{\smash-}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash-}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\rightarrow}
\makeatother

\makeatletter
\def \Rightarrowfill{\m@th\mathord{\smash=}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash=}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\Rightarrow}
\makeatother

\makeatletter
\def \midrightarrowfill{\m@th\mathord{\smash{\raisebox{.2ex}{$\scriptscriptstyle\mid$}}\!\!\,-}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash-}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\rightarrow}
\makeatother

\makeatletter
\def \midRightarrowfill{\m@th\mathord{\smash{\raisebox{.1ex}{$\scriptstyle\mid$}}\!\!\!=}\mkern-6mu%
  \cleaders\hbox{$\mkern-2mu\mathord{\smash=}\mkern-2mu$}\hfill
  \mkern-6mu\mathord\Rightarrow}
\makeatother

\newcommand{\overstackrel}[2]{\mathrel{\mathop{#1}\limits^{#2}}}
\newcommand{\trans}[1]{\mathbin{\smash[t]{\overstackrel{\rightarrowfill}{\ #1\ }}}}
\newcommand{\wtrans}[1]{\mathbin{\smash[t]{\overstackrel{\Rightarrowfill}{\ #1\ }}}} 
%% displaystyle version, without smashing
\newcommand{\dwtrans}[1]{\mathbin{{\overstackrel{\Rightarrowfill}{\ #1\ }}}} 
\newcommand{\ptrans}[1]{\mathbin{\smash[t]{\overstackrel{\midrightarrowfill}{\raisebox{-0.4ex}[0ex][-0.4ex]{$\scriptstyle\ #1\ $}}}}}
\newcommand{\dptrans}[1]{\mathbin{{\overstackrel{\midrightarrowfill}{{\raisebox{-0.4ex}[0ex][-0.4ex]{$\scriptstyle\ #1\ $}}}}}}

\newcommand{\tfg}[2][{}]{\llbracket {#2} \rrbracket_{#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shadows}
\usepackage{subcaption}
%% large arrows
\tikzset{
  big stealth/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=2*\scale]{stealth}}},
    postaction={decorate},
    shorten >=0.4pt}}
\tikzset{
  big ring/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{o}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big disc/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{*}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big box/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{open square}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big tile/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{square}}},
    postaction={decorate},
    shorten >=8pt*\scale}}

%% states
\tikzstyle{state}=[circle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=40pt]
%% places
\tikzstyle{place}=[circle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=40pt]
\tikzstyle{bplace}=[circle, very thick, fill, top color=cyan, fill
opacity=0.2, text opacity=1, bottom color=white, draw=cyan, minimum size=40pt]
% transitions
\tikzstyle{trans}=[rectangle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=32pt]
\tikzstyle{btrans}=[rectangle, very thick, fill, top color=cyan, fill
opacity=0.2, text opacity=1, bottom color=white, draw=cyan, minimum size=32pt]
%% arcs
\tikzstyle{arc}=[thick, big stealth, black]
\tikzstyle{barc}=[thick, big stealth, cyan]
\tikzstyle{read}=[thick, big disc, black]
\tikzstyle{inhibitor}=[thick, big ring, black]
\tikzstyle{stopwatch}=[thick, big tile, black]
\tikzstyle{stopwatchinhibitor}=[thick, big box, black]
\tikzstyle{priority}=[thick, big stealth, orange]
\tikzstyle{enabling}=[thick, big disc, orange]
\tikzstyle{disabling}=[thick, big ring, orange]
%% token
\tikzstyle{token}=[circle, fill, draw=black, minimum size=4pt]
%% glob options
\tikzstyle{glob-options}=[label
distance=6pt*\scalenodes*\scale,x=1pt,y=-1pt,scale=\scale,every
node/.style={transform shape}, baseline=(current bounding box.center)]
%% virtual node
\tikzstyle{virtual}=[circle, draw=white, minimum size=20pt]

%% TFGs
\usetikzlibrary{arrows.meta}
\tikzstyle{tnode}=[circle, thick, fill, top color=white, bottom color=white, draw=black, minimum size=30pt]
\tikzstyle{tred} = [thick, -{To}{Circle}]
\tikzstyle{tagg} = [thick, {Circle[open]}-{To}]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\scale{0.57}
\def\scalenodes{1.0}
\newcommand{\REGLE}[6]{
  \begin{figure}[p]
    \centering
    \begin{center}
      \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{
        \begin{minipage}[c]{1.0\linewidth}
          \vspace{1em} \noindent\textbf{\large{#1}}\\[1em]
          {#2}\\[1em]
        \end{minipage}}\\
        \hline & \\
        \begin{minipage}{.47 \textwidth} \begin{center}{#3}
          \end{center}
        \end{minipage} & \begin{minipage}{.47
            \textwidth} \begin{center}{#4}
          \end{center}
        \end{minipage}\\[1em]
        {$N_1$} & {$N_2$}\\[1em]
        \hline & \\
        \textbf{Condition}: {#5} & \textbf{Equation}: {#6}\\
               & \\
        \hline
      \end{tabular}
    \end{center}
    \caption{Rule {#1}}
  \end{figure}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tikz_header.tex <==
\usepackage{subcaption}

\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shadows}
%% large arrows
\tikzset{
  big stealth/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=2*\scale]{stealth}}},
    postaction={decorate},
    shorten >=0.4pt}}
\tikzset{
  big ring/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{o}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big disc/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{*}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big box/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{open square}}},
    postaction={decorate},
    shorten >=8pt*\scale}}
\tikzset{
  big tile/.style={
    decoration={markings,mark=at position -(0.1pt) with {\arrow[scale=1.5*\scale]{square}}},
    postaction={decorate},
    shorten >=8pt*\scale}}

%% states
\tikzstyle{state}=[circle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=40pt, drop shadow]
%% places
\tikzstyle{place}=[circle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=40pt, drop shadow]
\tikzstyle{bplace}=[circle, very thick, fill, top color=cyan, fill
opacity=0.2, text opacity=1, bottom color=white, draw=cyan, minimum size=40pt]
% transitions
\tikzstyle{trans}=[rectangle, very thick, fill, top color=white, bottom color=white, draw=black, minimum size=32pt, drop shadow]
\tikzstyle{btrans}=[rectangle, very thick, fill, top color=cyan, fill
opacity=0.2, text opacity=1, bottom color=white, draw=cyan, minimum size=32pt]
%% arcs
\tikzstyle{arc}=[thick, big stealth, black]
\tikzstyle{barc}=[thick, big stealth, cyan]
\tikzstyle{read}=[thick, big disc, black]
\tikzstyle{inhibitor}=[thick, big ring, black]
\tikzstyle{stopwatch}=[thick, big tile, black]
\tikzstyle{stopwatchinhibitor}=[thick, big box, black]
\tikzstyle{priority}=[thick, big stealth, orange]
\tikzstyle{enabling}=[thick, big disc, orange]
\tikzstyle{disabling}=[thick, big ring, orange]
%% token
\tikzstyle{token}=[circle, fill, draw=black, minimum size=4pt]
%% glob options
\tikzstyle{glob-options}=[label
distance=6pt*\scalenodes*\scale,x=1pt,y=-1pt,scale=\scale,every
node/.style={transform shape}, baseline=(current bounding box.center)]
%% virtual node
\tikzstyle{virtual}=[circle, draw=white, minimum size=20pt]

%% TFGs
\usetikzlibrary{arrows.meta}
\tikzstyle{tnode}=[circle, thick, fill, top color=white, bottom color=white, draw=black, minimum size=30pt]
\tikzstyle{tred} = [thick, -{To}{Circle}]
\tikzstyle{tagg} = [thick, {Circle[open]}-{To}]

%% Architecture
\tikzset{block/.style={draw, thick, text width=2.2cm, minimum height=1.5cm, align=center}, line/.style={-latex}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\conc}{\ensuremath{\mathbin{\|}}}

\newcommand{\caesar}{\textsc{c{\ae}sar.bdd}}
\newcommand{\kong}{\textsc{Kong}}
\newcommand{\reduce}{\textsc{Reduce}}
\newcommand{\sift}{\textsc{Sift}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

